Fine-Grained Buy-Many Mechanisms Are Not Much Better Than Bundling

Multi-item revenue-optimal mechanisms are known to be extremely complex, often offering buyers randomized lotteries of goods. In the standard buy-one model, it is known that optimal mechanisms can yield revenue infinitely higher than that of any "simple" mechanism -- the ones with size polynomial in the number of items -- even with just two items and a single buyer (Briest et al. 2015, Hart and Nisan 2017). We introduce a new parameterized class of mechanisms, buy-$k$ mechanisms, which smoothly interpolate between the classical buy-one mechanisms and the recently studied buy-many mechanisms (Chawla et al. 2019, Chawla et al. 2020, Chawla et al. 2022). Buy-$k$ mechanisms allow the buyer to buy up to $k$ many menu options. We show that restricting the seller to the class of buy-$n$ incentive-compatible mechanisms suffices to overcome the bizarre, infinite revenue properties of the buy-one model. Our main result is that the revenue gap with respect to bundling, an extremely simple mechanism, is bounded by $O(n^2)$ for any arbitrarily correlated distribution $\mathcal{D}$ over $n$ items for the case of an additive buyer. Our techniques also allow us to prove similar upper bounds for arbitrary monotone valuations, albeit with an exponential factor in the approximation. On the negative side, we show that allowing the buyer to purchase a small number of menu options does not suffice to guarantee sub-exponential approximations, even when we weaken the benchmark to the optimal buy-$k$ deterministic mechanism. If an additive buyer is only allowed to buy $k = \Theta(n^{1/2-\varepsilon})$ many menu options, the gap between the revenue-optimal deterministic buy-$k$ mechanism and bundling may be exponential in $n$. In particular, this implies that no "simple" mechanism can obtain a sub-exponential approximation in this regime.

==> TwoItemsTwoTickets.tex <==
\section{Warm-up: Proof of Theorem~\ref{thm:MainTwo}}
\label{sec:warmup}

In this section we will prove Theorem~\ref{thm:MainTwo}, restated here for convenience. 

\thmMainTwo*

As highlighted in the introduction of the paper, the proof of Theorem~\ref{thm:MainTwo} will be via the surrogate quantity, $\MenuGapTwo{2}{X}{Q}$. We will first show that for any distribution over two items $\distD$, there exists two sequences of points $(X, Q)$ such that $\MenuGapTwo{2}{X}{Q}$ upper bounds the ratio between the revenue-optimal buy-two mechanism for $\distD$ and the revenue from bundling, up to a constant factor (Lemma~\ref{lem:LB22}). Next we will show that this quantity itself is upper bounded for \emph{all} pairs of sequences $(X,Q)$ by another constant (Lemma~\ref{lem:UB22}). The proof of Theorem~\ref{thm:MainTwo} will then follow directly from Lemmas~\ref{lem:LB22},~\ref{lem:UB22}. 

\begin{lemma}
\label{lem:LB22}
For any distribution $\distD$ over $2$ items, there exists a sequence of points $X = \{\vec{x}_i\}_{i\geq1}$, $Q = \{\vec{q}_i\}_{i\geq0}$ (starting with $\vec{q}_0 = (0,0)$) such that 
$$ \MenuGapTwo{2}{X}{Q} \geq \frac{\btworev{\distD}}{20 \cdot \brev{\distD}}.$$
\end{lemma}

The second piece of the proof is to upper bound this quantity itself. 

\begin{lemma}
\label{lem:UB22}
For all sequences $X, Q$ as defined in Definition~\ref{def:main} it holds that $\MenuGapTwo{2}{X}{Q} \leq 2$.
\end{lemma}

\begin{proof}[Proof of Theorem~\ref{thm:MainTwo}]
Follows directly from Lemmas~\ref{lem:LB22},~\ref{lem:UB22}. 
\end{proof}

We devote the remainder of this section to the proofs of Lemmas~\ref{lem:LB22},~\ref{lem:UB22}.

\subsection{Proof of Lemma~\ref{lem:LB22}}

The proof of Lemma~\ref{lem:LB22} is split into two parts. In the first part, we will take the revenue-optimal buy-two menu for $\distD$ and massage it down to a sub-menu of interest whose buy-two revenue remains close to the optimal one. The sub-menu itself may not be buy-two incentive compatible. The key lies in \emph{only} removing menu entries, not altering existing ones. This does not change the incentive structure for the buyers whose options have remain intact. In the second part, we will show how to use that appropriate sub-menu in order to construct the desired sequence of points. The proof of Lemma~\ref{lem:LB22} follows the blueprint of a similar lemma for the buy-one case from~\cite{PSW22}. 

\subsubsection{Finding a sub-menu of Interest}

Let $\mech^* = \{(p_i, \vec{q}_i)\}_{i=1}$ be the revenue-optimal buy-two incentive-compatible menu, where $(p_i,\vec{q}_i)$ denotes the price and expected allocation of the $i$-th entry of the menu.  

\begin{claim}
\label{cl:disc2}
Let $\mech$ be a buy-two incentive compatible mechanism, $\mech_c \subseteq \mech$ be the sub-menu of $\mech$ that only offers options of price at least $c$. Then $\btworev{\distD, \mech_c} \geq \btworev{\distD, \mech}-c$. 
\end{claim}

\begin{proof}
If a buyer with valuation $\vec{v}$ chose a menu entry $(p,\vec{q})$ from the original menu $\mech$ with $p \geq c$, they will purchase the same menu entry in $\mech_c$ since $(p,\vec{q})$ was utility-maximizing and no new menu entries were introduced. If $p < c$, it is possible that the buyer would purchase some other option $(p', \vec{q}')$ (or combination of options). Regardless, the loss in revenue from that buyer is bounded by $c f(\vec{v})$. Let $S_c$ be the set of valuation vectors that preferred a menu entry in $\mech$ priced at $p < c$. Then the total loss in revenue is at most $c \sum_{\vec{v} \in S_c} f(\vec{v}) \leq c$.  
\end{proof}

\begin{claim}
\label{cl:split2}
Let $\mech$ be a mechanism whose prices are all at least $c$, and let $\mech_1, \mech_2 \subseteq \mech$ be sub-menus of $\mech$ defined as follows: 

\begin{itemize}
    \item $\mech_1$ has all menu entries whose price $p_i \in \cup_{i=0}^{\infty} [c \cdot 3^{2i}, c\cdot 3^{2i+1})$. 
    \item $\mech_2$ has all menu entries whose price $p_i \in \cup_{i=0}^{\infty} [c \cdot 3^{2i+1}, c \cdot 3^{2i+2})$. 
\end{itemize}
Then $\max_{i=1,2} \btworev{\distD, \mech_i} \geq \btworev{\distD, \mech}/2$.

\end{claim}

\begin{proof}
Because $\mech_1 \cup \mech_2 = \mech$, observe that 
$$\btworev{\distD, \mech} \leq \btworev{\distD, \mech_1} + \btworev{\distD, \mech_2}.$$ This is because any buyer with valuation $\vec{v}$ who purchases an option from $\mech_1$ when presented the menu $\mech$ will buy the same option when only presented $\mech_1$. By a simple averaging argument, the better of the two menus must get revenue at least half of the revenue of the original menu.  
\end{proof}

\begin{lemma}
\label{lem:menu2}
There exists a menu $\mech$ such that 

\begin{itemize}
    \item All prices are at least $c$.
    \item All prices belong to the union of intervals $\bigcup_{i=0}^{\infty} [ c \cdot 3^{2i+a}, c \cdot 3^{2i+a+1})$ for an $a \in \{0,1\}$.
    \item $\btworev{\distD, \mech} \geq \frac{\btworev{\distD}-c}{2}$. 
\end{itemize}

\end{lemma}

\begin{proof}
Take the revenue-optimal buy-two menu $\mech^*$, apply Claim~\ref{cl:disc2} to obtain a menu $\mech'$ that satisfies the first bullet point. Take the menu $\mech'$ and apply Claim~\ref{cl:split2} to obtain a menu $\mech$ that immediately satisfies the first and second bullet points. Finally, due to the revenue guarantees of Claims~\ref{cl:disc2},~\ref{cl:split2}, we have that $\btworev{\distD, \mech} \geq \frac{\btworev{\distD, \mech'}}{2} \geq \frac{\btworev{\distD}-c}{2}$. 
\end{proof}

We will eventually choose $c = O(\btworev{\distD})$. Thus at this point we have shown that there will always exist a somewhat structured sub-menu whose buy-two revenue is approximately optimal. The menu itself may not be buy-two incentive compatible. 

\subsubsection{Construction of the Sequences $X, Q$}

In this subsection we will show how to use the sub-menu found in the previous subsection to construct the sequences $(X,Q)$ of interest who would witness $\MenuGapTwo{2}{X}{Q} \geq O\left(\btworev{\distD}/\brev{\distD}\right)$. 

Consider the menu $\mech$ from Lemma~\ref{lem:menu2}. Let $\mathcal{B}_j \subseteq \mech$ be the sub-menu that has all menu entries priced in $[3^{2j+a}, 3^{2j+a+1})$ for the same $a \in \{0, 1\}$ from Lemma~\ref{lem:menu2}. Let $\vec{x}_j$ be a valuation on $\mathcal{B}_j$ such that $|\vec{x}_j|_1 \leq (1+\delta) |\vec{x}|_1$ for all $\vec{x} \in \mathcal{B}_j$. We call such a valuation the \emph{representative of bin} $\mathcal{B}_j$. Let $X$ be the sequence defined by representatives and $Q$ be the sequence defined by the respective allocations $\vec{q}_j \in \mech$ of each representative $\vec{x}_j$, with $\vec{q}_0 = \vec{0}$.  

We now prove a series of claims that will allow us to prove the main result of this subsection. The first claim simply upper bounds the probability of sampling a vector from each bin as a function of the norm of the representative and $\brev{\distD}$, the benchmark of interest. 

\begin{claim}
\label{cl:bundleprob2}
$\Pr(\vec{x} \in \mathcal{B}_j) \leq \frac{\brev{\distD}(1+\delta)}{|\vec{x}_j|_1}$.
\end{claim}

\begin{proof}
Consider the mechanism that sells the grand bundle at price $|\vec{x}_j|_1/(1+\delta)$. Since any valuation on $\mathcal{B}_j$ has value at least that much for the grand bundle, the revenue of this menu is at least $\Pr(\vec{x} \in \mathcal{B}_j) |\vec{x}_j|_1/(1+\delta)$. But this is a grand bundling menu and is thus its revenue is at most $\brev{\distD}$. 
\end{proof}

The next claim lower bounds the gap contribution of the $j$-th representative as a function of parameters from Claim~\ref{cl:bundleprob2} as well as the price $p_j$ of the menu entry that allocates $\vec{q}_j$. 

\begin{claim}
\label{cl:gap2}
$\frac{\gaptwo{2}{j}{X}{Q}}{|\vec{x}_j|_1} \geq \frac{\Pr(\vec{x} \in \mathcal{B}_j) p_j}{3 \cdot \brev{\distD} (1+\delta)}$. 
\end{claim}

\begin{proof}
Because the initial mechanism $\mech^*$ was buy-two incentive-compatible, we know that for any pair of options $\vec{q}_{j'}, \vec{q}_{j''}$,  

$$ \vec{x}_j \cdot \vec{q}_j - p_j \geq \vec{x}_j \cdot \lottery(\vec{q}_{j'}, \vec{q}_{j''}) - p_{j'} - p_{j''}.$$

We can rewrite this as 

$$ \frac{\gaptwo{2}{j}{X}{Q}}{|\vec{x}_j|_1} \geq \frac{p_j - p_{j'} - p_{j''}}{|\vec{x}_j|_1} \geq \frac{p_j}{(3\cdot |\vec{x}_j|_1)} \geq \frac{\Pr(\vec{x} \in \mathcal{B}_j) p_j}{3 \cdot \brev{\distD} (1+\delta)}.$$ 

Recall by our choice of points and the fact that $j', j'' < j$, $p_j \geq 3 \cdot p_{j'}, 3 \cdot p_{j''}$. Thus, the second inequality follows. The third inequality follows from Claim~\ref{cl:bundleprob2} since we have that $\frac{1}{|\vec{x}_j|_1} \geq \frac{\Pr(\vec{x} \in \mathcal{B}_j) p_j}{\brev{\distD} (1+\delta)}$.

\end{proof}

We are now ready to prove Lemma~\ref{lem:LB22}. 

\begin{proof}[Proof of Lemma~\ref{lem:LB22}] 

Let us first observe the following fact

\begin{equation}
\label{eq:pricegap}
 \btworev{\distD, \mech} = \sum_j \sum_{\vec{x} \in \mathcal{B}_j} p(x) f(x) \leq \sum_j \Pr(\vec{x} \in \mathcal{B}_j) 3 p_j.
\end{equation}
 
Recall that for any valuation $\vec{x} \in \mathcal{B}_j$, its price $p(\vec{x})$ is no greater than $3 p_j$. Therefore, the inequality follows. Moreover, from Claim~\ref{cl:gap2} we get that 

\begin{equation}
\label{eq:gap2lb}
\MenuGapTwo{2}{X}{Q} = \sum_j \gaptwo{2}{j}{X}{Q} \geq \sum_j \frac{ \Pr(\vec{x} \in \mathcal{B}_j)p_j}{3 \cdot \brev{\distD} (1+\delta)}.
\end{equation}


Applying Eqn.~\ref{eq:pricegap} together with Lemma~\ref{lem:menu2} we get that
\begin{equation}
\label{eq:gap2ub}
\sum_j \Pr(\vec{x} \in \mathcal{B}_j) p_j \geq \btworev{\distD, \mech}/3 \geq (\btworev{\distD,}-c)/6. 
\end{equation}


Putting Eqns.~\ref{eq:gap2lb},~\ref{eq:gap2ub} we get that
\begin{equation} 
\label{eq:final2}
\MenuGapTwo{2}{X}{Q} \geq \frac{ (\btworev{\distD}-c)}{18\cdot \brev{\distD}(1+\delta)}.
\end{equation}

Let $c = \btworev{\distD}/100, \delta = 1/100$ in Eqn.~\ref{eq:final2}. Therefore, 

$$ \MenuGapTwo{2}{X}{Q} \geq \frac{99 \cdot \btworev{\distD}}{101\cdot 18\cdot \brev{\distD}} \geq \frac{\btworev{\distD}}{20\cdot  \brev{\distD}}.$$ 



\end{proof}

\subsection{Proof of Lemma~\ref{lem:UB22}}

Given a sequence of points $Q$, let $Q_i$  be the sequence truncated at the $i$-th point, that is to say $Q_i = \{\vec{q}_0, \vec{q}_1, ..., \vec{q}_i \}$. Let $\vec{m}_i = (\max_{\vec{q}_{i} \in Q_i} \{\vec{q}_{i,1}\}, \max_{\vec{q}_{i} \in Q_i} \{\vec{q}_{i,2}\})$ be the $2$-dimensional vector whose entries are the largest coordinates among the points in $Q_i$. 

\begin{claim}
\label{cl:maxgap2}
For any $i$, $\gaptwo{2}{i}{X}{Q}/||\vec{x}_i||_1 \leq \max \{\vec{q}_{i,1}-\vec{m}_{i-1,1}, 0\}+\max \{\vec{q}_{i,2}-\vec{m}_{i-1,2}, 0\}.$
\end{claim}

\begin{proof}
Let $\vec{x}_i, \vec{q}_i$ be given. Since $\gaptwo{2}{i}{X}{Q}$ is defined to be the minimum over all pairs of previously placed points, we can just upper bound it by witnessing its value with two earlier points. Let $i^*_1, i^*_2$ be the indices such that: 

\begin{itemize}
    \item $i^*_1, i^*_2 < i,$
    \item $\vec{q}_{i^*_1,1} = \vec{m}_{i-1,1},$
    \item $\vec{q}_{i^*_2,2} = \vec{m}_{i-1,2}.$
\end{itemize}

That is to say, $i^*_1, i^*_2$ are the indices of the points that witness that $\vec{m}_{i-1}$ is indeed the coordinate-wise maximum of all points in $Q_{i-1}$. Then 
\begin{equation}
\label{eq:gaptwoub2}
\frac{\gaptwo{2}{i}{X}{Q}}{||\vec{x}_i||_1} \leq \frac{\vec{x}_i}{||\vec{x_i}||_1} \cdot (\vec{q}_i - \lottery(\vec{q}_{i^*_1}, \vec{q}_{i^*_2})).
\end{equation}

Recall that 
\begin{align*}
\lottery(\vec{q}_{i^*_1}, \vec{q}_{i^*_2})_1 \geq \max\{\vec{q}_{i^*_1,1}, \vec{q}_{i^*_2,1}\} \geq \vec{m}_{i-1,1},\\   
\lottery(\vec{q}_{i^*_1}, \vec{q}_{i^*_2})_2 \geq \max\{\vec{q}_{i^*_1,2}, \vec{q}_{i^*_2,2}\} \geq \vec{m}_{i-1,2}.
\end{align*}

Therefore, 
\begin{align}
\label{eq:obsgap1}
\vec{q}_{i,1} - \lottery(\vec{q}_{i^*_1}, \vec{q}_{i^*_2})_1 \leq \vec{q}_{i,1} - \vec{m}_{i-1,1},\\
\label{eq:obsgap2}
\vec{q}_{i,2} - \lottery(\vec{q}_{i^*_1}, \vec{q}_{i^*_2})_2 \leq \vec{q}_{i,2} - \vec{m}_{i-1,2}.  
\end{align}


Therefore, for any choice of $\vec{x}_i$, it will be true that 
\begin{align*}
\frac{\gaptwo{2}{i}{X}{Q}}{||\vec{x}_i||_1} & \leq \frac{\vec{x}_i}{||\vec{x}_i||_1} \cdot (\vec{q}_i - \lottery(\vec{q}_{i^*_1}, \vec{q}_{i^*_2})) \\ 
& = \frac{\vec{x}_{i,1}}{||\vec{x}_i||_1} (\vec{q}_{i,1} - \lottery(\vec{q}_{i^*_1},\vec{q}_{i^*_2})_1) + \frac{\vec{x}_{i,2}}{||\vec{x}_i||_1} (\vec{q}_{i,2} - \lottery(\vec{q}_{i^*_1},\vec{q}_{i^*_2})_2) \\ 
& \leq \frac{\vec{x}_{i,1}}{||\vec{x}_i||_1} (\vec{q}_{i,1} - \vec{m}_{i-1,1}) + \frac{\vec{x}_{i,2}}{||\vec{x_i}||_1} (\vec{q}_{i,2} - \vec{m}_{i-1,2}) \\
& \leq \max\{0, \vec{q}_{i,1} - \vec{m}_{i-1,1}\} + \max\{0, \vec{q}_{i,2} - \vec{m}_{i-1,2}\}.  
\end{align*}
\end{proof}
With Claim~\ref{cl:maxgap2} at hand, the proof of Lemma~\ref{lem:UB22} will follow easily. 
\begin{proof}[Proof of Lemma~\ref{lem:UB22}]
For any pair of sequences $(X,Q)$,  
\begin{align*}
\MenuGapTwo{2}{X}{Q} & = \sum_{i=1}^N \gaptwo{2}{i}{X}{Q}/||x_i||_1 \\ 
& \leq \sum_{i=1}^N (\max \{\vec{q}_{i,1}-\vec{m}_{i-1,1}, 0\})+\sum_{i=1}^N (\max \{\vec{q}_{i,2}-\vec{m}_{i-1,2}, 0\}) \\
& \leq \sum_{i=1}^N  (\vec{m}_{i,1}-\vec{m}_{i-1,1}) + \sum_{i=1}^N  (\vec{m}_{i,2}-\vec{m}_{i-1,2}) \\
& \leq 2. 
\end{align*}

The first inequality follows from Claim~\ref{cl:maxgap2}. For the second inequality, first note that by definition $\vec{q}_{i,1} \leq \vec{m}_{i,1}$, with equality only if $\vec{q}_{i,1} \geq \vec{q}_{i',1}$ for all $i' < i$. But note also that by definition $\vec{m}_{i,1}-\vec{m}_{i-1,1} \geq 0$. Therefore $\max \{\vec{m}_{i,1}-\vec{m}_{i-1,1}, 0 \} \leq \vec{m}_{i,1}-\vec{m}_{i-1,1}$. The last inequality follows from observing that the final sum across each coordinate telescopes. Since $\vec{q}_{i,1} \leq 1$, the sum is at most $1$ per coordinate. 

\end{proof}

\begin{observation}
Setting both sequences $(X,Q)$ equal to the standard basis of $\mathbb{R}^2$ shows that Lemma~\ref{lem:UB22} is tight.
\end{observation}

